Easy Begun is Half Done: Spatial-Temporal Graph Modeling with ST-Curriculum Dropout

Spatial-temporal (ST) graph modeling, such as traffic speed forecasting and taxi demand prediction, is an important task in deep learning area. However, for the nodes in graph, their ST patterns can vary greatly in difficulties for modeling, owning to the heterogeneous nature of ST data. We argue that unveiling the nodes to the model in a meaningful order, from easy to complex, can provide performance improvements over traditional training procedure. The idea has its root in Curriculum Learning which suggests in the early stage of training models can be sensitive to noise and difficult samples. In this paper, we propose ST-Curriculum Dropout, a novel and easy-to-implement strategy for spatial-temporal graph modeling. Specifically, we evaluate the learning difficulty of each node in high-level feature space and drop those difficult ones out to ensure the model only needs to handle fundamental ST relations at the beginning, before gradually moving to hard ones. Our strategy can be applied to any canonical deep learning architecture without extra trainable parameters, and extensive experiments on a wide range of datasets are conducted to illustrate that, by controlling the difficulty level of ST relations as the training progresses, the model is able to capture better representation of the data and thus yields better generalization.

==> Formulation.tex <==





==> Related_work.tex <==
\noindent\textbf{Curriculum Learning.}
% The basic idea of curriculum learning is to let models first learn from easy samples and work their way up to complex samples and knowledge \cite{bengio2009curriculum}. Recently, this concept has been extended with the research effort in this area. \cite{soviany2021curriculum} summarizes the taxonomy of curriculum learning into data-level and model-level. The data-level approach follows the natural definition of curriculum learning through sampling \cite{jiang2014easy}, weighting \cite{kumar2010self} and specific iterative \cite{spitkovsky2009baby}. The other bunch of study focus on progressively increasing the model's capacity. For example, \cite{karras2017progressive} designs a novel training strategy by gradually increasing the model's capacity via adding new neural units. \cite{sinha2020curriculum} combines the idea of adversarial training with curriculum learning by using Gaussian kernel to smooth the noise in CNN feature maps at early stages of training. \cite{morerio2017curriculum} introduces the dynamically stochastic dropout in curriculum learning by moderately enlarging the dropout rate during training.
The basic idea of curriculum learning is to let the models first learn from easy samples and work their way up to complex samples and knowledge \cite{bengio2009curriculum}. A well-written survey \cite{wang2021survey} classifies the taxonomy of curriculum learning into data-level and criteria-level. The data-level approach follows the natural definition of curriculum learning through sampling \cite{jiang2014easy}, weighting \cite{kumar2010self} and specific iterative \cite{spitkovsky2009baby} to select the most suitable examples for each training step. The other bunch of study considers arranging the curriculum according to some criteria which can be any design element in training a machine learning model. A novel training strategy \cite{karras2017progressive} has been designed to gradually increase the model's capacity by adding new neural units. Reference \cite{sinha2020curriculum} combines the idea of adversarial training with curriculum learning by using Gaussian kernel to smooth the noise in CNN feature maps at early stages of training. Reference \cite{morerio2017curriculum} introduces the dynamically stochastic dropout in curriculum learning by moderately increasing the dropout rate during training to handle co-adaptions in DNN. 

% Motivated by these work, this paper aims to bring the idea of curriculum learning into spatial-temporal graph modeling. On ST graph, the learning difficulty of each node can vary greatly, causing the model to suffer from both the over-fitting of easy nodes and the failure to model complex nodes. This has become one of bottlenecks for the state-of-the-arts models while CL can alleviate such situation. Therefore, we propose a simple plug-in for ST models to perform CL without extra trainable parameters, which can automatically detect the difficult samples in ST model’s training procedure.



\noindent\textbf{Spatial-temporal Graph Modeling.}
The task of spatial-temporal graph modeling intends to forecast the future single/multi step signals according to the historical observation and spatial graph information. Lots of applications including taxi demand prediction \cite{yang2021dual}, human action recognition \cite{peng2020learning} and traffic speed forecast \cite{wu2020connecting} can be categorized to this case. Meanwhile, different types of RNN-based and CNN-based models, such as \cite{seo2018structured} and \cite{yan2018spatial}, have been developed to solve the task of spatial-temporal graph modeling. 
% For example, \cite{peng2020learning} designs a neural architecture search framework to automatically design GCN structure for the task of human action recognition.
% \cite{yu2017spatio} designs a complete convolutional structure via integrating the graph neural network and  1D convolution to model the problem of traffic forecast. 
% Despite there are lots of methods proposed, but in literature, seldom effort concentrated on the learning tactics in spatial-temporal graph. To the best of our knowledge, we are the first to propose the curriculum learning-based approach in spatial-temporal graph modeling. 
% The  spatial-temporal outliers detection  also an importance researching directions. For example,  \cite{liu2011discovering} builds the outlier causality trees to spatio-temporal outliers in traffic data, and discover the potential flaws designs in road network.  \cite{zhang2019decomposition} finds out the abnormal flow by decomposing urban dynamics into normal and abnormal component. However, in literature, seldom work pay attention to the learning procedure of graph neural network, which may suffer from unstable result caused by disorder knowledge in model. In this paper, we combine the outlier detection into the training precess to encourage the easy pattern exposed in model earlier, and gradually increasing pattern's complexity. 

%\section{Crowd Flow Prediction}
%The  crowd flows prediction is a very important research topic in spatial-temporal data mining, and large parts of ST-models have been proposed and  widely deployed in the government to manage the traffic and protect public safety. \cite{zhang2016dnn} firstly proposes the deep learning-based  model,  which  solves  the  problem  by  combining  convolutional neural network (CNN) and deep neural networks (DNN). \cite{zhang2017deep} further defines the time series concept of the  recent time intervals, daily periodicity, and weekly trend patterns  and  uses  the  ResNet \cite{he2016deep}. A branch of work \cite{yao2019revisiting,lin2019deepstn+,zonoozi2018periodic} improve the performance based on the framework on \cite{zhang2017deep}. However, existing technologies have also been subjected to criticism regarding their lack of an efficient training strategy for the characteristic of human flow, since the flow prediction task involved multiple complex patterns, and easily to disturb the model's knowledge in earlier training stage. 


%\begin{table*}[h]
%	\centering
%	\footnotesize
%	\caption{ Effectiveness Evaluation on TaxiBJ and TaxiNYC }\label{tab:result1}
%	\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
%		\hline & \multicolumn{5}{|c|} { \textbf{TaxiBJ} } & \multicolumn{5}{|c|} { \textbf{TaxiNYC} } \\
%		\hline Model & MSE & RMSE & MAE  & MAPE & Improved & MSE & RMSE & MAE & MAPE & Improved \\
%		\hline 
%		CNN & $520.525$ & $22.815$ & $12.995$ & $8.46 \%$ &$\backslash$ & $243.360$ & $15.600$ & $6.122$ & $8.08 \%$&$\backslash$ \\
%		CNN+Drop & 526.336&  22.942&  13.519 & $8.46 \%$ &$\backslash$ & 248.618&  15.768&   6.280  & $8.24 \%$&$\backslash$ \\
%		CNN+STDrop  & $512.237$ & $22.632$ & $12.701$ & $8.27 \%$ &$\backslash$ & 239.411&  15.473&   6.036 & $7.88 \%$&$\backslash$ \\
%		\hline
%		ST-ResNet & 369.937&  19.234&  10.936 & $8.46 \%$ &$\backslash$ & 135.104&  11.623&   5.182 & $8.08 \%$&$\backslash$ \\
%		ST-ResNet+Drop & 381.090 &  19.522&  11.295 & $8.46 \%$ &$\backslash$ & 159.614&  12.634&   5.151 & $8.08 \%$&$\backslash$ \\
%		ST-ResNet+STDrop & 356.188&  18.873&  10.738 & $8.46 \%$ &$\backslash$ & 130.824&  11.438&   5.049 & $8.08 \%$&$\backslash$ \\
%		
%		\hline
%	\end{tabular}
%	
%\end{table*}
%However, \cite{morerio2017curriculum} are designed on the task of image classification by alleviating the phenomenon of   co-adaptations within feature detectors.  
